LMLT: Low-to-high Multi-Level Vision Transformer for Image Super-Resolution

Recent Vision Transformer (ViT)-based methods for Image Super-Resolution have demonstrated impressive performance. However, they suffer from significant complexity, resulting in high inference times and memory usage. Additionally, ViT models using Window Self-Attention (WSA) face challenges in processing regions outside their windows. To address these issues, we propose the Low-to-high Multi-Level Transformer (LMLT), which employs attention with varying feature sizes for each head. LMLT divides image features along the channel dimension, gradually reduces spatial size for lower heads, and applies self-attention to each head. This approach effectively captures both local and global information. By integrating the results from lower heads into higher heads, LMLT overcomes the window boundary issues in self-attention. Extensive experiments show that our model significantly reduces inference time and GPU memory usage while maintaining or even surpassing the performance of state-of-the-art ViT-based Image Super-Resolution methods. Our codes are availiable at https://github.com/jwgdmkj/LMLT.

==> tex/sec3_fig2_mechanism.tex <==
%%%%%% Figure 3 : Concept of Multi-level %%%%%%
%--------------------------------------------------------
\begin{figure*}[!t]\footnotesize
 \begin{center}
  \begin{tabular}{ccccccc}
    \multicolumn{3}{c}{\multirow{5}*[53pt]{
        \includegraphics[width=0.3\linewidth, height=0.33\linewidth]{picture/others/window_show.pdf}}} &\hspace{-3.5mm}
      \includegraphics[width=0.15\linewidth, height = 0.15\linewidth]{picture/others/butterfly.pdf} &\hspace{-2mm}
      \includegraphics[width=0.15\linewidth, height = 0.15\linewidth]{picture/others/butt_head0.pdf} &\hspace{-2mm}
      \includegraphics[width=0.15\linewidth, height = 0.15\linewidth]{picture/others/butt_head1.pdf} &\hspace{-2mm}
      \includegraphics[width=0.15\linewidth, height = 0.15\linewidth]{picture/others/butt_head2.pdf} \\
      \multicolumn{3}{c}{~} &\hspace{-3.5mm}  &\hspace{-3.5mm}(a) 1st Head &\hspace{-3.5mm}(b) 2nd Head &\hspace{-3.5mm}(c) 3rd Head \\

      \multicolumn{3}{c}{~} & \hspace{-3.5mm}
      & \hspace{-2mm}
      \includegraphics[width=0.15\linewidth, height = 0.15\linewidth]{picture/others/butt_head3.pdf} & \hspace{-2mm}
      \includegraphics[width=0.15\linewidth, height = 0.15\linewidth]{picture/others/butt_aggr.pdf} & \hspace{-2mm}
      \includegraphics[width=0.15\linewidth, height = 0.15\linewidth]{picture/others/butt_final.pdf} \\
      \multicolumn{3}{c}{\hspace{-3.5mm} } & &\hspace{-3.5mm}(d) 4th Head   &\hspace{-3.5mm}(e) Aggregated &\hspace{-3.5mm}(f) Attended
      
\\
 \end{tabular}
 \end{center}
 % \vspace{-2mm}
 \caption{\textbf{Left} Self-attention(SA) at different spatial resolutions of the image with the same window size. The colors originally indicate the same area. Performing self-attention on a larger area allows each head to receive additional information from outside its own region, enabling access to a relatively wider area. \textbf{Right} Features from each head. (a) to (d) are the features from the first to the fourth head, respectively. (e) is after aggregation, and (f) is after applying activation and then multiplying with the original feature.}
 \label{fig:mechanism}
\end{figure*}

==> tex_table/sec4_tab2_base.tex <==
%---------------------60 dim experiment-------------------------
\begin{table}[t]
	\caption{Comparisons with our LMLT-Base and other Super-Resolution models on multiple benchmark datasets. Best and second-best performance are in \textcolor{red}{red} and \textcolor{blue}{blue} color, and third-best performance is in \underline{underlined} respectively.}
	\label{tab:base}
	\renewcommand\arraystretch{1.1}
	\begin{center}
		\resizebox{\textwidth}{!}{
			\begin{tabular}{| c | c | c | c | c | c | c | c | c |}
				\hline
				Scale & Method & \#Params & \#FLOPs & Set5 & Set14 & B100 & Urban100 & Manga109 \\
				\hline
            % -------- X2 60
				\multirow{8}*{$\times 2$} 
                & IMDN ~\cite{IMDN}  &694K   &156G  & 38.00/0.9605 & 33.63/0.9177 & 32.19/0.8996 & 32.17/0.9283 & 38.88/0.9774 \\
				~ & LatticeNet~\cite{Lattice}    &756K   &170G   & \underline{38.06}/0.9607 & 33.70/0.9187 & 32.20/0.8999 & 32.25/0.9288  & 38.94/0.9774 \\
				~ & RFDN-L ~\cite{rfdn}  &626K   &146G  & \textcolor{blue}{38.08}/0.9606  & 33.67  /0.9190  & 32.18/0.8996  & 32.24/0.9290  & 38.95/0.9773 \\
				~ & SRPN-Lite~\cite{srpn}       &609K  &140G  &\textcolor{red}{38.10}/\underline{0.9608} & 33.70/0.9189 & 32.25/0.9005& 32.26/0.9294 & -  \\
				~ & HNCT ~\cite{hnct}       &357K     &82G & \textcolor{blue}{38.08}/\underline{0.9608}  & 33.65/0.9182  & 32.22/0.9001  & 32.22/0.9294  & 38.87/0.9774 \\
				~ & FMEN~\cite{fmen}  &748K     &172G  & \textcolor{red}{38.10}/\textcolor{blue}{0.9609}  & \underline{33.75}/\underline{0.9192}  & \underline{32.26}/\underline{0.9007}  & \underline{32.41}/\underline{0.9311}  & \underline{38.95}/\textcolor{blue}{0.9778} \\
				~ & NGswin(~ \cite{ngswin}    &990K     &140G &38.05/\textcolor{red}{0.9610} & \textcolor{red}{33.79}/\textcolor{blue}{0.9199} & \textcolor{blue}{32.27}/\textcolor{blue}{0.9008} & \textcolor{red}{32.53}/\textcolor{red}{0.9324} & \textcolor{blue}{38.97}/\underline{0.9777} \\
                ~ & \textbf{LMLT-Base(Ours)} & 652K & 158G  & \textcolor{red}{38.10}/\textcolor{red}{0.9610} & \textcolor{blue}{33.76}/\textcolor{red}{0.9201} & \textcolor{red}{32.28}/\textcolor{red}{0.9012} & \textcolor{blue}{32.52}/\textcolor{blue}{0.9316} & \textcolor{red}{39.24}/\textcolor{red}{0.9783} \\
                
				\hline
            % -------- X3 60
				\multirow{8}*{$\times 3$} 
                & IMDN ~\cite{IMDN}         &703K     &72G  & 34.36/0.9270 & 30.32/0.8417 & 29.09/0.8046 & 28.17/0.8519 & 33.61/0.9445 \\
				~ & LatticeNet~\cite{Lattice}           &765K   &76G   &34.40/0.9272 & 30.32/0.8416 & 29.10/0.8049 & 28.19/0.8513 & 33.63/0.9442 \\
				~ & RFDN-L( ~\cite{rfdn}  &633K   &66G   &\underline{34.47}/\underline{0.9280}  &30.35/0.8421  &29.11/0.8053  &28.32/0.8547  &33.78/0.9458 \\
				~ & SRPN-Lite~\cite{srpn}       &615K    &63G  & \underline{34.47}/\underline{0.9280} & 30.38/0.8425 & 29.16/0.8061 & 28.22/0.8534 & - \\
				~ & HNCT ~\cite{hnct}       &363K     &38G & \underline{34.47}/0.9275  & \textcolor{blue}{30.44}/\underline{0.8439}  & 29.15/\underline{0.8067}  & 28.28/0.8557  & 33.81/0.9459 \\
				~ & FMEN~\cite{fmen}  &757K     &77G  &34.45/0.9275  & \underline{30.40}/0.8435  & \underline{29.17}/0.8063  & \underline{28.33}/\underline{0.8562}  & \underline{33.86}/\underline{0.9462} \\
				~ & NGswin~\cite{ngswin}           &1,007K     &67G  & \textcolor{blue}{34.52}/\textcolor{blue}{0.9282} & \textcolor{red}{30.53}/\textcolor{blue}{0.8456} & \textcolor{blue}{29.19}/\textcolor{blue}{0.8078} & \textcolor{red}{28.52}/\textcolor{red}{0.8603} & \textcolor{blue}{33.89}/\textcolor{blue}{0.9470} \\

                ~ & \textbf{LMLT-Base(Ours)} & 660K & 75G  & \textcolor{red}{34.58}/\textcolor{red}{0.9285} & \textcolor{red}{30.53}/\textcolor{red}{0.8458} & \textcolor{red}{29.21}/\textcolor{red}{0.8084} & \textcolor{blue}{28.48}/\textcolor{blue}{0.8581} & \textcolor{red}{34.18}/\textcolor{red}{0.9477} \\
				\hline
    
            % -------- X4 60
				\multirow{8}*{$\times 4$} 
                & IMDN ~\cite{IMDN}         &715K     &41G & 32.21/0.8948 & 28.58/0.7811 & 27.56/0.7353 & 26.04/0.7838 & 30.45/0.9075 \\
				~ & LatticeNet~\cite{Lattice}           &777K   &44G   & 32.18/0.8943 & 28.61/0.7812 & 27.57/0.7355 & 26.14/0.7844 & 30.54/0.9075 \\
				~ & RFDN-L ~\cite{rfdn}  &643K   &38G  & 32.28/0.8957 & 28.61/0.7818 & 27.58/0.7363 & 26.20/0.7883 & 30.61/0.9096 \\
                ~ & SRPN-Lite~\cite{srpn}       &623K    &36G  & 32.24/\underline{0.8958} & 28.69/\underline{0.7836} & \underline{27.63}/0.7373 & 26.16/0.7875 & - \\
				~ & HNCT ~\cite{hnct}       &373K     &22G & \underline{32.31}/0.8957  & \underline{28.71}/0.7834  & \underline{27.63}/\underline{0.7381}  & 26.20/0.7896  & \underline{30.70}/\underline{0.9112} \\
				~ & FMEN~\cite{fmen}  &769K     &44G & 32.24/0.8955  & 28.70/\textcolor{blue}{0.7839}  & \underline{27.63}/0.7379  & \underline{26.28}/\underline{0.7908}  & \underline{30.70}/0.9107 \\
				~ & NGswin~\cite{ngswin}           &1,019K     &36G & \textcolor{blue}{32.33}/\textcolor{blue}{0.8963} &\textcolor{blue}{28.78}/\textcolor{red}{0.7859} & \textcolor{blue}{27.66}/\textcolor{blue}{0.7396} & \textcolor{red}{26.45}/\textcolor{red}{0.7963} &  \textcolor{blue}{30.80}/\textcolor{blue}{0.9128} \\
                ~ & \textbf{LMLT-Base(Ours)} & 672K & 41G & \textcolor{red}{32.38}/\textcolor{red}{0.8971} & \textcolor{red}{28.79}/\textcolor{red}{0.7859} & \textcolor{red}{27.70}/\textcolor{red}{0.7403} & \textcolor{blue}{26.44}/\textcolor{blue}{0.7947} & \textcolor{red}{31.09}/\textcolor{red}{0.9139} \\
				\hline
		\end{tabular}}
	\end{center}
% \vspace{-3mm}
\end{table}
%--------------------------------------------------------

==> tex_table/sec4_tab3_large.tex <==
%---------------------84 chan exp-------------------------
\begin{table}[t]
	\caption{Comparisons with our LMLT-Large and other Super-Resolution models on multiple benchmark datasets. Best and second-best performance are in \textcolor{red}{red} and \textcolor{blue}{blue} color.}
	\label{tab:large}
	\renewcommand\arraystretch{1.1}
	\begin{center}
		\resizebox{\textwidth}{!}{
			\begin{tabular}{| c | c | c | c |  c | c | c | c | c |}
				\hline
				Scale & Method & \#Params & \#FLOPs & Set5 & Set14 & B100 & Urban100 & Manga109 \\
				\hline
    
            % -------- X2 84
				\multirow{5}*{$\times 2$} 
                & ESRT~\cite{esrt}        & 751K & - &38.03/0.9600&33.75/0.9184&32.25/0.9001&32.58/0.9318&39.12/0.9774\\
				~ & SwinIR-light~\cite{SwinIR}     &910K & 244G  &38.14/0.9611&33.86/0.9206&32.31/0.9012&\textcolor{blue}{32.76}/\textcolor{blue}{0.9340}&39.12/0.9783 \\
                ~ & ELAN~\cite{elan} &621K &203G &38.17/0.9611&\textcolor{blue}{33.94}/0.9207&32.30/0.9012&\textcolor{blue}{32.76}/\textcolor{blue}{0.9340}&39.11/0.9782 \\ 
                ~ &SRformer-Light~\cite{srformer}       & 853K & 236G & \textcolor{red}{38.23}/\textcolor{red}{0.9613}&\textcolor{blue}{33.94}/\textcolor{blue}{0.9209}&\textcolor{red}{32.36}/\textcolor{red}{0.9019}&\textcolor{red}{32.91}/\textcolor{red}{0.9353}&\textcolor{blue}{39.28}/\textcolor{blue}{0.9785} \\ 
                ~ & \textbf{LMLT-Large(Ours)} & 1,270K & 306G& \textcolor{blue}{38.18}/\textcolor{blue}{0.9612} & \textcolor{red}{33.96}/\textcolor{red}{0.9212} & \textcolor{blue}{32.33}/\textcolor{blue}{0.9017} & 32.75/0.9336 & \textcolor{red}{39.41}/\textcolor{red}{0.9786} \\
				\hline

                % -------- X3 84
    		  \multirow{5}*{$\times 3$} 
                & ESRT~\cite{esrt}    & 751K & - &34.42/0.9268&30.43/0.8433&29.15/0.8063&28.46/0.8574&33.95/0.9455\\
                ~ & SwinIR-light~\cite{SwinIR}   &918K & 111G &34.62/0.9289&30.54/0.8463&29.20/0.8082&28.66/0.8624&33.98/0.9478 \\
                ~ & ELAN~\cite{elan} &629K &90G &34.61/0.9288&30.55/0.8463&\textcolor{blue}{29.21}/0.8081&28.69/0.8624&34.00/0.9478 \\ 
                ~ &SRformer-Light~\cite{srformer}  & 861K & 105G & \textcolor{red}{34.67}/\textcolor{red}{0.9296}&\textcolor{blue}{30.57}/\textcolor{blue}{0.8469}&\textcolor{red}{29.26}/\textcolor{red}{0.8099}&\textcolor{red}{28.81}/\textcolor{red}{0.8655}&\textcolor{blue}{34.19}/\textcolor{blue}{0.9489} \\
                ~ & \textbf{LMLT-Large(Ours)} & 1,279K & 144G& \textcolor{blue}{34.64}/\textcolor{blue}{0.9293} & \textcolor{red}{30.60}/\textcolor{red}{0.8471} & \textcolor{red}{29.26}/\textcolor{blue}{0.8097} & \textcolor{blue}{28.72}/\textcolor{blue}{0.8626} & \textcolor{red}{34.43}/\textcolor{red}{0.9491} \\
    		\hline
    
            % -------- X4 84
				\multirow{5}*{$\times 4$}
                & ESRT~\cite{esrt}  & 751K & - &32.19/0.8947&28.69/0.7833&27.69/0.7379&26.39/0.7962&30.75/0.9100\\
				~ & SwinIR-light~\cite{SwinIR}  &930K & 64G &32.44/0.8976&28.77/0.7858&27.69/0.7406&26.47/0.7980&30.92/0.9151 \\
				~ & ELAN~\cite{elan} &640K &54G &32.43/0.8975&28.78/0.7858&27.69/0.7406&26.54/0.7982&30.92/0.9150 \\ 
                ~ &SRformer-Light~\cite{srformer}  & 873K & 63G & \textcolor{red}{32.51}/\textcolor{red}{0.8988} &\textcolor{blue}{28.82}/\textcolor{blue}{0.7872} &\textcolor{blue}{27.73}/\textcolor{red}{0.7422}&\textcolor{red}{26.67}/\textcolor{red}{0.8032}&\textcolor{blue}{31.17}/\textcolor{red}{0.9165}\\
                ~ & \textbf{LMLT-Large(Ours)} & 1,295K & 78G& \textcolor{blue}{32.48}/\textcolor{blue}{0.8987} & \textcolor{red}{28.87}/\textcolor{red}{0.7879} & \textcolor{red}{27.75}/\textcolor{blue}{0.7421} & \textcolor{blue}{26.63}/\textcolor{blue}{0.8001} & \textcolor{red}{31.32}/\textcolor{blue}{0.9163} \\
				\hline
		\end{tabular}}
	\end{center}
% \vspace{-3mm}
\end{table}
%--------------------------------------------------------
